An absolute calibration of the near-infrared Period-Luminosity Relations of Type II Cepheids in the Milky Way and in the Large Magellanic Cloud

We present time-series photometry of 21 nearby Type II Cepheids in the near-infrared J, H and Ks passbands. We use this photometry, together with the Third Gaia Early Data Release parallaxes, to determine for the first time period-luminosity relations (PLRs) for Type II Cepheids from field representatives of these old pulsating stars in the near-infrared regime. We found PLRs to be very narrow for BL Herculis stars, which makes them candidates for precision distance indicators. We then use archival photometry and the most accurate distance obtained from eclipsing binaries to recalibrate PLRs for Type II Cepheids in the Large Magellanic Cloud (LMC). Slopes of our PLRs in the Milky Way and in the LMC differ by slightly more than 2{\sigma} and are in a good agreement with previous studies of the LMC, Galactic Bulge and Galactic Globular Clusters Type II Cepheids samples. We use PLRs of Milky Way Type II Cepheids to measure the distance to the LMC and we obtain a distance modulus of 18.540$\pm$0.026(stat.)$\pm$0.034(syst.)mag in the WJKs Wesenheit index. We also investigate the metallicity effect within our Milky Way sample and we find rather significant value of about -0.2mag/dex in each band meaning that more metal-rich Type II Cepheids are intrinsically brighter than their more metal-poor counterparts, in agreement with the value obtained from Type II Cepheids in Galactic Globular Clusters. The main source of systematic error on our Milky Way PLRs calibration and the LMC distance is the current uncertainty of the Gaia parallax zero point.

==> Makefile <==
### ====================================================================
### [30-Jul-2005]
### ====================================================================

prefix		= /usr/local

CP		= /bin/cp -p

INSTDIRS	= $(prefix)/share/lib/tex/inputs \
		  $(prefix)/share/lib/tex/latex \
		  $(prefix)/share/lib/tex/latex2e/unpacked

LATEX		= latex
LATEX		= latex2e

LN		= /bin/ln -f

LS		= ls

RM		= /bin/rm -f

SHELL		= /bin/sh

TEX		= tex

### ====================================================================

LTXFILES	= tepsf2.ltx

TEXFILES	= tepsf1.tex  tepsf3.tex

### ====================================================================

all:
	@echo There is nothing to build in this directory.

check:	check-latex check-tex

check-latex:
	for f in $(LTXFILES) ; \
	do \
		$(LATEX) $$f ; \
		$(LS) -l `basename $$f .ltx`.* ; \
	done

check-tex:
	for f in $(TEXFILES) ; \
	do \
		$(TEX) $$f ; \
		$(LS) -l `basename $$f .tex`.* ; \
	done

clean:
	-$(RM) *.aux
	-$(RM) *.dvi
	-$(RM) *.log
	-$(RM) *~
	-$(RM) \#*
	-$(RM) a.out
	-$(RM) core core.*

clobber:	distclean

distclean:	mostlyclean

maintainer-clean:	distclean
	@echo "This command is intended for maintainers to use;"
	@echo "it deletes files that may require special tools to rebuild."

mostlyclean: clean

install:	uninstall
	for d in $(INSTDIRS) ; \
	do \
		$(CP) epsf.tex $$d/epsf.tex ; \
		$(LN) $$d/epsf.tex $$d/epsf.sty ; \
	done

uninstall:
	for d in $(INSTDIRS) ; \
	do \
		$(RM) $$d/epsf.tex $$d/epsf.sty ; \
	done


==> tepsf1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Preamble

\input epsf.tex

\def \bs {\char`\\}

\def \heading #1{\centerline{\bf #1}}

\def \myfont {%
    \baselineskip = 9.6pt
    \font \rm = cmr8 at 8pt
    \rm
}

\def \noise
{%
    Blah blah blah blah blah blah. Blah blah blah blah blah blah. Blah
    blah blah blah blah blah. Blah blah blah blah blah blah
}

\def \ARROWPICTURE {\llap{$\Rightarrow$}\PLAINPICTURE\rlap{$\Leftarrow$}}

\def \PLAINPICTURE {\epsffile{tepsf.eps}}

\parindent = 2em

\parskip = 2ex plus 0.5ex minus 0.5ex

%% Page size in mid-Atlantic units
\voffset = -0.5in

\vsize = 9.5in

\hsize = 12.5cm

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Document body

\myfont

\heading{Test of {\tt epsf.tex}}

\noise

This figure should be centered:

\centerline{\PLAINPICTURE}

\noise

This figure should be left-adjusted:

\leftline{\PLAINPICTURE}

\noise

This figure should be right-adjusted:

\rightline{\PLAINPICTURE}

\noise

This figure should be centered with abutting arrows on the baseline:

\centerline{\ARROWPICTURE}

\noise

This figure should be left-adjusted with abutting arrows on the
baseline, the leftmost of which is in the left margin on the baseline:

\leftline{\ARROWPICTURE}

\noise

This figure should be right-adjusted with abutting arrows on the
baseline, the rightmost of which is in the right margin on the
baseline:

\rightline{\ARROWPICTURE}

\noise

\vfill
\eject

%% ---------------------------------------------------------------------

\heading{Test of {\tt epsf.tex}}
\heading{with}
\heading{{\tt \bs epsfframetrue} and {\tt \bs epsfshowfalse} and
         {\tt \bs epsfshowfilenametrue}}

\epsfframetrue
\epsfshowfalse
\epsfshowfilenametrue
\epsfverbosetrue

\noise

This figure should be centered:

\centerline{\PLAINPICTURE}

\noise

This figure should be left-adjusted:

\leftline{\PLAINPICTURE}

\noise

This figure should be right-adjusted:

\rightline{\PLAINPICTURE}

\noise

This figure should be centered with abutting arrows on the baseline:

\centerline{\ARROWPICTURE}

\noise

This figure should be left-adjusted with abutting arrows on the
baseline, the leftmost of which is in the left margin on the baseline:

\leftline{\ARROWPICTURE}

\noise

This figure should be right-adjusted with abutting arrows on the
baseline, the rightmost of which is in the right margin on the
baseline:

\rightline{\ARROWPICTURE}

\noise

\vfill
\eject

%% ---------------------------------------------------------------------

\bye


==> tepsf3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Preamble

\input epsf.tex

\def \bs {\char`\\}

\def \heading #1{\centerline{\bf #1}}

\def \myfont {%
    \baselineskip = 9.6pt
    \font \rm = cmr8 at 8pt
    \rm
}

\def \noise
{%
    Blah blah blah blah blah blah. Blah blah blah blah blah blah. Blah
    blah blah blah blah blah. Blah blah blah blah blah blah
}

\def \ARROWPICTURE {\llap{$\Rightarrow$}\PLAINPICTURE\rlap{$\Leftarrow$}}

\def \PLAINPICTURE {\epsffile{tepsf.eps}}

\parindent = 2em

\parskip = 2ex plus 0.5ex minus 0.5ex

%% Page size in mid-Atlantic units
\voffset = -0.5in

\vsize = 9.5in

\hsize = 12.5cm

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Document body

\myfont

\heading{Test of {\tt epsf.tex}}

\noise

This figure should be centered:

\centerline{XXX\vbox{\PLAINPICTURE}XXX}

\noise

This figure should be left-adjusted:

\leftline{\vbox{\PLAINPICTURE}XXX}

\noise

This figure should be right-adjusted:

\rightline{XXX\vbox{\PLAINPICTURE}}

\noise

This figure should be centered:

\centerline{XXX\hbox{\PLAINPICTURE}XXX}

\noise

This figure should be left-adjusted:

\leftline{\hbox{\PLAINPICTURE}XXX}

\noise

This figure should be right-adjusted:

\rightline{XXX\hbox{\PLAINPICTURE}}

\noise

This figure should be centered with abutting arrows on the baseline:

\centerline{\vbox{\ARROWPICTURE}}

\noise

This figure should be left-adjusted with abutting arrows on the
baseline, the leftmost of which is in the left margin on the baseline:

\leftline{\vbox{\ARROWPICTURE}}

\noise

This figure should be right-adjusted with abutting arrows on the
baseline, the rightmost of which is in the right margin on the
baseline:

\rightline{\vbox{\ARROWPICTURE}}

\noise

\vfill
\eject

%% ---------------------------------------------------------------------

\bye

